New evidence for the ubiquity of prominent polar dust emission in AGN on tens of parsec scales

The key ingredient of active galactic nuclei (AGN) unification, the dusty obscuring torus was so far held responsible for the observed mid-infrared (MIR) emission of AGN. However, the best studied objects with VLTI/MIDI show that instead a polar dusty wind is dominating these wavelengths, leaving little room for a torus contribution. But is this wind an ubiquitous part of the AGN? To test this, we conducted a straightforward detection experiment, using the upgraded VLT/VISIR for deep subarcsecond resolution MIR imaging of a sample of nine [O IV]-bright, obscured AGN, all of which were predicted to have detectable polar emission. Indeed, the new data reveal such emission in all objects but one. We further estimate lower limits on the extent of the polar dust and show that the polar dust emission is dominating the total MIR emission of the AGN. These findings support the scenario that polar dust is not only ubiquitous in AGN but also an integral part of its structure, processing a significant part of the primary radiation. The polar dust has to be optically thin on average, which explains, e.g., the small dispersion in the observed mid-infrared--X-ray luminosity correlation. At the same time, it has to be taken into account when deriving covering factors of obscuring material from mid-infrared to bolometric luminosity ratios. Finally, we find a new tentative trend of increasing MIR emission size with increasing Eddington ratio.

==> test.tex <==
\begin{table*}
\caption{Properties of the sample}
\label{tab:sam}
\centering
\begin{tabular}{l c c c c c c c c c c c c c}
\hline\hline
 & Opt. &  & intr. & $\log L$ & $\log L_\mathrm{intr.}$ &  &  &  &  & $\log F$ &  & SA & \\
Object & class & D & resol & $(12\um)$ & (2-10\,keV) & $\log \nh$ & $\log \mbh$ & Ref. & $\log \ledd$ & (\oiv) & Ref. & PA & Ref.\\
 &  & [Mpc] & [pc/as] & [erg/s] & [erg/s] & [cm$^{-2}$] & [$\msun$] &  &  & [erg/cm/s$^{2}$] &  & [deg] & \\
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) & (14)\\
\hline
3C321 & 2.0 & 460.0 & 1857 & 44.6 & 43.7 & 24.0 & \dots & \dots & \dots & -12.1 & 1 & 138 & 2, 3\\
IC4518W & 2.0 & 76.1 & 357 & 43.5 & 43.0 & 23.3 & \dots & \dots & \dots & -12.1 & 4 & 13 & 5\\
Mrk573 & 2.0 & 73.1 & 343 & 43.5 & 43.2 & $\ge$24.2 & \dots & \dots & \dots & -12.1 & 6 & 130 & 7, 8, 9, 10\\
NGC1365 & 1.8 & 17.9 & 87 & 42.5 & 42.1 & 23.2 & 7.3 & 11 & -2.25 & -11.8 & 12 & 125 & 13, 14, 15, 16, 17\\
NGC2110 & 2.0 & 35.9 & 172 & 43.1 & 42.7 & 22.5 & 8.7 & 11 & -3.16 & -12.3 & 18 & 171 & 19, 20, 21, 22\\
NGC5135 & 2.0 & 66.0 & 311 & 43.2 & 43.2 & 24.4 & 7.0 & 23 & -0.85 & -12.2 & 12 & 15 & 24, 25\\
NGC5506 & 1.9 & 31.6 & 151 & 43.4 & 43.1 & 22.4 & 7.6 & 11 & -1.59 & -11.7 & 12 & -13 & 26, 27\\
NGC5643 & 2.0 & 20.9 & 100 & 42.5 & \dots & $\ge$24.3 & 7.0 & 28 & \dots & -12.1 & 12 & 86 & 29, 30, 31\\
NGC7582 & 1.8 & 23.0 & 112 & 42.9 & 42.4 & 23.1 & 7.7 & 32 & -2.46 & -11.7 & 12 & 70 & 30, 15\\
\hline	
\end{tabular}

